Is Hierarchical Quantization Essential for Optimal Reconstruction?

Vector-quantized variational autoencoders (VQ-VAEs) are central to models that rely on high reconstruction fidelity, from neural compression to generative pipelines. Hierarchical extensions, such as VQ-VAE2, are often credited with superior reconstruction performance because they split global and local features across multiple levels. However, since higher levels derive all their information from lower levels, they should not carry additional reconstructive content beyond what the lower-level already encodes. Combined with recent advances in training objectives and quantization mechanisms, this leads us to ask whether a single-level VQ-VAE, with matched representational budget and no codebook collapse, can equal the reconstruction fidelity of its hierarchical counterpart. Although the multi-scale structure of hierarchical models may improve perceptual quality in downstream tasks, the effect of hierarchy on reconstruction accuracy, isolated from codebook utilization and overall representational capacity, remains empirically underexamined. We revisit this question by comparing a two-level VQ-VAE and a capacity-matched single-level model on high-resolution ImageNet images. Consistent with prior observations, we confirm that inadequate codebook utilization limits single-level VQ-VAEs and that overly high-dimensional embeddings destabilize quantization and increase codebook collapse. We show that lightweight interventions such as initialization from data, periodic reset of inactive codebook vectors, and systematic tuning of codebook hyperparameters significantly reduce collapse. Our results demonstrate that when representational budgets are matched, and codebook collapse is mitigated, single-level VQ-VAEs can match the reconstruction fidelity of hierarchical variants, challenging the assumption that hierarchical quantization is inherently superior for high-quality reconstructions.

==> sec/abstract.tex <==
\begin{abstract}


Vector Quantized VAEs (VQ-VAEs) have achieved remarkable success in learning discrete representations for images. A hierarchical variant, VQ-VAE2, has been shown to produce higher-fidelity reconstructions by capturing global and local features at multiple codebook levels. However, hierarchical models introduce complexity, and it remains unclear whether their gains stem from the multi-level architecture per se or simply from increased latent capacity and better codebook utilization. In this work, we perform a rigorous comparison between a two-level hierarchical VQ-VAE and a single-level “flat” VQ-VAE with matched capacity. We identify under-utilization of code vectors as a key factor limiting single-level VQ-VAE performance. By applying two simple strategies to mitigate codebook collapse (code embedding initialization and periodic refresh of unused code vectors), we show that a flat VQ-VAE can attain reconstruction quality on par with a hierarchical VQ-VAE. Our flat model, given the same number of latent dimensions and codebook size as the hierarchical model, achieves comparable mean squared error (MSE) and perceptual quality on the ImageNet dataset. We further analyze the effect of codebook dimensionality on learning, finding that extremely high-dimensional code embeddings hinder effective usage. Our results suggest that, with proper training techniques, single-level VQ-VAEs are capable of matching hierarchical VQ-VAEs in reconstruction fidelity, challenging the prevailing view that hierarchy is indispensable for VQ-VAE performance.

\end{abstract}
